Constraining the systematics of (acoustic) wave heating estimates in the solar chromosphere

Acoustic wave heating is believed to contribute significantly to the missing energy input required to maintain the solar chromosphere in its observed state. We studied the propagation of waves above the acoustic cutoff in the upper photosphere into the chromosphere with ultraviolet and optical spectral observations interpreted through comparison with three dimensional radiative magnetohydrodynamic (rMHD) \emph{Bifrost} models to constrain the heating contribution from acoustic waves in the solar atmosphere. Sit-and-stare observations taken with the Interface Region Imaging Spectrograph (IRIS) and data from the Interferometric BIdimensional Spectrograph (IBIS) were used to provide the observational basis of this work. We compared the observations with synthetic observables derived from the Bifrost solar atmospheric model. Our analysis of the \emph{Bifrost} simulations show that internetwork and enhanced network regions exhibit significantly different wave propagation properties, which are important for the accurate wave flux estimates. The inferred wave energy fluxes based on our observations are not sufficient to maintain the solar chromosphere. We point out that the systematics of the modeling approaches in the literature lead to differences which could determine the conclusions of this type of studies, based on the same observations.

==> Sections/Mu_dependence.tex <==
\section{Wave power dependence on observing  inclination angle}
\label{sec:Mu_dependence}

\subsection{Plage}

\subsection{Coronal holes}

\subsection{Quiet Sun}
